Sleeping Model: Local and Dynamic Algorithms

In recent years the sleeping model came to the focus of researchers. In this model nodes can go into a sleep state in which they spend no energy but at the same time cannot receive or send messages, nor can they perform internal computations. This model captures energy considerations of a problem. A problem P is an O-LOCAL problem if, given an acyclic orientation on the edges of the input graph, one can solve the problem as follows. Each vertex awaits the decisions of its parents according to the given orientation and can make its own decision in regard to P using only the information about its parents decisions. problems and showed that for this class of problems there is a deterministic algorithm that runs in $O(\log \Delta)$ awake time. The clock round complexity of that algorithm is $O(\Delta^2)$. In this work we offer three algorithms for the bf O-LOCAL class of problems with a trade off between awake complexity and clock round complexity. One of these algorithms requires only $O(\Delta^{1+\epsilon})$ clock rounds for some constant $\epsilon>0$ but still only $O(\log \Delta)$ awake time which improves on the algorithm in \cite{BM21}. We add to this two other algorithms that trade a higher awake complexity for lower clock round complexity. We note that the awake time incurred is not that significant. We offer dynamic algorithms in the sleeping model. We show three algorithms for solving dynamic problems in the O-LOCAL class as well as an algorithm for solving any dynamic decidable problem. We show that one can solve any {\bf O-LOCAL} problem in constant awake time in graphs with constant neighborhood independence. Specifically, our algorithm requires $O(K)$ awake time where $K$ is the neighborhood independence of the input graph. Graphs with bounded neighborhood independence are well studied with several results in recent years for several core problem in the distributed setting.

==> CHANGELOG <==
LIPICS Style - CHANGELOG

* 10/12/2018 LIPIcs-v2019 v2.0
** New Features
*** support of metadata in PDF file (e.g. author, title, keywords) 
*** revised displaying of author-related funding acknowledgements (now displayed as part of the funding block instead of footnotes)
*** added support for cleveref package (new document option 'cleveref')
*** added support for using autoref for theorem-like environments (new document option 'autoref')
*** added new environment claim and claimproof to realize sub-proofs
*** added new environment proposition
** Bugfixes
*** fixed problems with theorem-like environments when using cleveref and autoref (see new features above)
*** switched several URL from http to https
*** fixed problems with using of ACM 2012 classification (deactivated subjclass and revised support of ccsdesc macro)
** Minor changes
*** moved ORCID symbol behind author name (according https://orcid.org/content/journal-display-guidelines)
*** added separator \and to split several affiliations
*** added warnings when package 'enumitem' or 'paralist' are loaded; they manipulate the pre-defined enumeration styles and are partly incompatible
*** preloaded package 'microtype' in style
*** revised spacings/font sizes for top matter

* 09/04/2018 LIPIcs-v2018 v1.5
** Bugfixes
*** Fixed problem with page style in case of many authors
*** Fixed aggregation of authors for ToC file

* 15/03/2018 LIPIcs-v2018 v1.4
** Bugfixes
*** Fixed enumerations
*** Fixed aggregation of authors for ToC file

* 26/02/2018 LIPIcs-v2018 v1.3
** Bugfixes
*** Fixed \hideLIPIcs
*** Fixed enumerations
*** Fixed typo
** Revised display of ORCIDs following recommendation by ORCID

* 06/02/2018 LIPIcs-v2018 v1.2
** Release of LIPIcs-v2018
*** revised author macro \author{name}{affil}{email}{orcid}{funding} 
*** added support for ORCIDs
*** switched to ACM 2012 classification system
*** added new macros for extended metadata \category, \relatedversion, \supplement, \funding, \acknowledgements
*** added warnings for missing mandatory metadata
*** added preconfigured enumeration styles based on the enumerate package
*** added option \hideLIPIcs to hide all LIPIcs related information
*** added support for line numbers
** Bugfixes
*** fixed copyright line
*** added warning when using outdated subfig package due to incompatibilities in preloaded subcaption package
*** fixed bug when using MnSymbol package
*** fixed bug in numbering in theorem-like environments used in appendix
*** fixed problems in ToC file

